Knowledge Graph Prompting for Multi-Document Question Answering

The `pre-train, prompt, predict' paradigm of large language models (LLMs) has achieved remarkable success in open-domain question answering (OD-QA). However, few works explore this paradigm in the scenario of multi-document question answering (MD-QA), a task demanding a thorough understanding of the logical associations among the contents and structures of different documents. To fill this crucial gap, we propose a Knowledge Graph Prompting (KGP) method to formulate the right context in prompting LLMs for MD-QA, which consists of a graph construction module and a graph traversal module. For graph construction, we create a knowledge graph (KG) over multiple documents with nodes symbolizing passages or document structures (e.g., pages/tables), and edges denoting the semantic/lexical similarity between passages or intra-document structural relations. For graph traversal, we design an LLM-based graph traversal agent that navigates across nodes and gathers supporting passages assisting LLMs in MD-QA. The constructed graph serves as the global ruler that regulates the transitional space among passages and reduces retrieval latency. Concurrently, the graph traversal agent acts as a local navigator that gathers pertinent context to progressively approach the question and guarantee retrieval quality. Extensive experiments underscore the efficacy of KGP for MD-QA, signifying the potential of leveraging graphs in enhancing the prompt design for LLMs. Our code: https://github.com/YuWVandy/KG-LLM-MDQA.

==> production.tex <==
% \section*{Production Application}
% Here each question is paired with 10 documents with 2 documents including the evidence and the other 8 documents negatively sampled. The evaluation metrics consist of the accuracy, the number of tokens for the fetched contexts and the answers.

% \begin{table*}[]
% \centering
% \begin{tabular}{l|ccc|ccc|ccc|ccc}
% \hline
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{HotpotQA}} & \multicolumn{3}{c|}{\textbf{IIRC}} & \multicolumn{3}{c|}{\textbf{WikiMhop}} & \multicolumn{3}{c}{\textbf{DocInstruct}} \\

%  & Acc & EM & F1 & Acc & EM & F1 & Acc & EM & F1 & Acc & EM & F1 \\
% \hline
% None & 43.06 & 19.32 & 31.15 & 19.96 & 8.19 & 13.00 & 41.48 & 18.64 & 25.10 \\
% \hline
% KNN & 72.08 & 40.63 & 58.40 & 45.55 & 25.64 & 37.32 & 50.21 & 31.28 & 41.59 &  &  &  \\
% TF-IDF & \textbf{76.46} & \textbf{45.83} & \textbf{64.54} & 48.94 & 26.69 & 40.21 & 56.21 & 34.62 & 44.77 &  &  & \\
% BM25 & 72.88 & 42.44 & 60.51 & 42.16 & 24.58 & 36.17 & 54.55 & 29.96 & 39.76 &  & \\
% \hline
% IRCoT &  &  &  &  &  &  &  &  &  &  &  &  \\
% LLM-KG & 74.84 & 44.99 & 64.44 & \textbf{50.96} & \textbf{28.05} & \textbf{42.16} & \textbf{61.35} & \textbf{38.21} & \textbf{49.85} \\
% \hline
% Golden & 82.69 & 50.31 & 71.36 & 65.97 & 35.92 & 54.95 & 70.88 & 40.36 & 59.68\\
% \hline
% \end{tabular}
% \caption{Main Performance}
% \end{table*}


%emphasize hallucination issue
%reinforcement the benefit
%tables and pages (some content below the bag-of-word table) in Figure 3
%Time complexity
%(1) Efficient, by increasing the number of negative documents
%(2) changing the graph construction parameter, check the performance
%(3) different LLM-guiddedd graph



\begin{table*}[]
\scriptsize
\centering
\begin{tabular}{lccccc|ccccc|ccccc}
\hline
\multirow{2}{*}{} & \multicolumn{5}{c|}{HotpotQA} & \multicolumn{5}{c|}{IIRC} & \multicolumn{5}{c}{WikiMultiHop} \\
 & @1 & @5 & @10 & @20 & @30 & @1 & @5 & @10 & @20 & @30 & @1 & @5 & @10 & @20 & @30 \\
\hline
KNN\_Fuzzy & 4.95 & 23.74 & 42.35 & 67.47 & 69.16 & 3.04 & 18.10 & 32.78 & 49.56 & 51.91 & 5.91 & 33.71 & 52.85 & 64.52 & 65.98 \\
TF-IDF & 27.04 & 64.55 & 78.01 & 85.47 & 87.58 & 28.41 & 50.52 & 57.03 & 64.48 & 67.31 & 20.04 & 50.07 & 59.94 & 67.60 & 72.67 \\
BM25 & 24.01 & 57.39 & 67.30 & 74.28 & 77.02 & 19.60 & 36.56 & 41.79 & 47.87 & 51.00 & 13.14 & 37.70 & 46.78 & 54.43 & 58.28 \\
DPR &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
MDR &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
Ours &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline
\end{tabular}
\caption{Retrieval Recall}
\end{table*}


\begin{table*}[]
\scriptsize
\centering
\begin{tabular}{lccccc|ccccc|ccccc}
\hline
\multirow{2}{*}{} & \multicolumn{5}{c|}{HotpotQA} & \multicolumn{5}{c|}{IIRC} & \multicolumn{5}{c}{WikiMultiHop} \\
 & @1 & @5 & @10 & @20 & @30 & @1 & @5 & @10 & @20 & @30 & @1 & @5 & @10 & @20 & @30 \\
\hline
KNN\_Fuzzy & 11.59 & 11.22 & 10.08 & 7.99 & 5.47 & 7.23 & 8.64 & 7.91 & 5.97 & 4.18 & 13.07 & 15.73 & 12.61 & 7.71 & 5.24 \\
TF-IDF & 63.09 & 30.56 & 18.52 & 10.25 & 7.01 & 65.19 & 24.39 & 13.82 & 7.80 & 5.44 & 47.65 & 23.48 & 14.07 & 8.02 & 5.79 \\
BM25 & 55.93 & 26.78 & 15.90 & 8.84 & 6.11 & 45.22 & 17.20 & 9.85 & 5.66 & 4.03 & 31.83 & 17.58 & 11.07 & 6.50 & 4.69 \\
DPR &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
MDR &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
Ours &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline
\end{tabular}
\caption{Retrieval Precision}
\end{table*}


\begin{table*}[]
\scriptsize
\centering
\begin{tabular}{lccccc|ccccc|ccccc}
\hline
\multirow{2}{*}{} & \multicolumn{5}{c|}{HotpotQA} & \multicolumn{5}{c|}{IIRC} & \multicolumn{5}{c}{WikiMultiHop} \\
 & @1 & @5 & @10 & @20 & @30 & @1 & @5 & @10 & @20 & @30 & @1 & @5 & @10 & @20 & @30 \\
\hline
KNN\_Fuzzy & 0 & 6.00 & 17.18 & 40.99 & 42.65 & 0.21 & 4.04 & 11.06 & 22.55 & 24.04 & 0 & 12.66 & 27.17 & 38.59 & 39.63 \\
TF-IDF & 0 & 31.96 & 53.20 & 67.22 & 71.13 & 0.63 & 15.82 & 23.63 & 33.76 & 38.19 & 0 & 20.86 & 32.92 & 42.13 & 49.90 \\
BM25 & 0 & 26.40 & 38.25 & 50.73 & 54.68 & 0.21 & 8.07 & 12.10 & 18.68 & 21.44 & 0 & 14.37 & 21.77 & 28.54 & 32.65 \\
DPR &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
MDR &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
Ours & 0 & 26.34 & 56.43 &  &  &  &  &  &  &  &  &  &  &  &  \\
\hline
\end{tabular}
\caption{Retrieval EM}
\end{table*}


% \begin{table*}[]
% \centering
% \begin{tabular}{l|ccc|ccc|ccc|ccc}
% \hline
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{HotpotQA}} & \multicolumn{3}{c|}{\textbf{IIRC}} & \multicolumn{3}{c|}{\textbf{WikiMhop}} & \multicolumn{3}{c}{\textbf{DocStruct}} \\

%  & EM & Acc & F1 & EM & Acc & F1 & EM & Acc & F1 & EM & Acc & F1 \\
%  \hline
% Nei &  &  &  &  & &  &  &  &  &  &  &  \\
% Nei$_1$ &  &  &  &  & &  &  &  &  &  &  &  \\
% Nei$_2$ &  &  &  &  & &  &  &  &  &  &  &  \\
% \hline
% RW &  &  &  &  &  &  &  &  &  &  &  & \\
% RW$_1$ &  &  &  &  &  &  &  &  &  &  &  & \\
% RW$_2$ &  &  &  &  &  &  &  &  &  &  &  & \\
% \hline
% Ours &  &  & &  \\
% \hline
% \end{tabular}
% \caption{Ablation Performance}
% \end{table*}



% \begin{table}[htbp!]
% \caption{Ablation study}
% \centering
% \begin{tabular}{l|ccc|ccc}
% \hline
% \multirow{2}{*}{Method} & \multicolumn{3}{c|}{HotpotQA - 100 Qs} & \multicolumn{3}{c}{Internal Data} \\
%  & Acc & \# Token & \# Ans Token & Acc & \# Token & \# Ans Token \\
% \hline
% KNN + Fuzzy Search & 59.79 & 1404.86 & 4.13 &  &  &  \\
% \hline
% MultiGraph + Neighbors & 66.67 & 1467.84 & 4.24 &  &  &  \\
% MultiGraph + Emb Ranked Neighbors & 62.63 & 1130.74 & 4.17 &  &  &  \\
% MultiGraph + Text Ranked Neighbors & 62.50 & 1418.10 & 4.39 &  &  &  \\
% \hline
% MultiGraph + RW & 63.92 & 1467.52 & 4.31 &  &  &  \\
% MultiGraph + Emb Ranked RW & 62.63 & 1483.42 & 4.13 &  &  &  \\
% MultiGraph + Text Ranked RW & 63.16 & 1418.31 & 4.46 &  &  &  \\
% \hline
% Retrieval & 68.00 & 1212.23 & 4.24 &  &  &  \\
% MultiGraph + Retrieval & 68.37 & 1486.10 & 4.06 &  &  & \\
% \hline
% \end{tabular}
% \end{table}











% \begin{table}[htbp!]
% \caption{Ablation study}
% \centering
% \begin{tabular}{l|ccc|ccc}
% \hline
% \multirow{2}{*}{Method} & \multicolumn{3}{c|}{HotpotQA - 100 Qs} & \multicolumn{3}{c}{Internal Data} \\
%  & Acc & \# Token & \# Ans Token & Acc & \# Token & \# Ans Token \\
% \hline
% KNN + Fuzzy Search & 59.79 & 1404.86 & 4.13 &  &  &  \\
% \hline
% MultiGraph + Neighbors & 66.67 & 1467.84 & 4.24 &  &  &  \\
% MultiGraph + Emb Ranked Neighbors & 62.63 & 1130.74 & 4.17 &  &  &  \\
% MultiGraph + Text Ranked Neighbors & 62.50 & 1418.10 & 4.39 &  &  &  \\
% \hline
% MultiGraph + RW & 63.92 & 1467.52 & 4.31 &  &  &  \\
% MultiGraph + Emb Ranked RW & 62.63 & 1483.42 & 4.13 &  &  &  \\
% MultiGraph + Text Ranked RW & 63.16 & 1418.31 & 4.46 &  &  &  \\
% \hline
% Retrieval & 68.00 & 1212.23 & 4.24 &  &  &  \\
% MultiGraph + Retrieval & 68.37 & 1486.10 & 4.06 &  &  & \\
% \hline
% \end{tabular}
% \end{table}

